Rotationally Equivariant 3D Object Detection

Rotation equivariance has recently become a strongly desired property in the 3D deep learning community. Yet most existing methods focus on equivariance regarding a global input rotation while ignoring the fact that rotation symmetry has its own spatial support. Specifically, we consider the object detection problem in 3D scenes, where an object bounding box should be equivariant regarding the object pose, independent of the scene motion. This suggests a new desired property we call object-level rotation equivariance. To incorporate object-level rotation equivariance into 3D object detectors, we need a mechanism to extract equivariant features with local object-level spatial support while being able to model cross-object context information. To this end, we propose Equivariant Object detection Network (EON) with a rotation equivariance suspension design to achieve object-level equivariance. EON can be applied to modern point cloud object detectors, such as VoteNet and PointRCNN, enabling them to exploit object rotation symmetry in scene-scale inputs. Our experiments on both indoor scene and autonomous driving datasets show that significant improvements are obtained by plugging our EON design into existing state-of-the-art 3D object detectors.

==> figtext/overview_rebut.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/overview_v4.pdf}
    \vspace{-0.35cm}
    \caption{\scriptsize Updated main figure in the main paper.}
    \vspace{-0.6cm}
    \label{fig:rebut_overview}
\end{figure}

==> figtext/votenet.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/votenet.png}
    \caption{\ourvn: Our instantiation on VoteNet.}
    \label{fig:votenet}
\end{figure*}

==> tbltext/cmp_3rscan.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{c|cccccccccc|c}
        \toprule
        Method &  &  &  &  &  &  &  &  &  &  &  \\
        \hline
        VoteNet~\cite{}  \\
        \ourvn (ours)  \\
        \bottomrule
    \end{tabular}
    \caption{Performance comparison of VoteNet with and without our partially equivariant design on 3RScan dataset (IoU=25\%).}
    \label{tbl:cmp_3rscan}
\end{table*}

==> tbltext/cmp_scan2cad_256.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{c|cccccccccc|c}
        \toprule
        Method & Trash-bin & Display & Bathtub & Chair & Cabinet & Bookshelf & Table & Sofa & Bed & Others & mAP \\
        \hline
        VoteNet~\cite{} & 35.7 & 27.6 & 46.3 & 85.7 & 44.5 & 48.7 & 76.1 & \tb{66.4} & \tb{85.1} & 16.3 & 53.2 \\
        \ourvn (ours) & \tb{56.9} & \tb{32.8} & \tb{49.3} & \tb{86.5} & \tb{54.6} & \tb{51.3} & \tb{77.6} & 65.9 & 82.6 & \tb{21.5} & \tb{57.9} \\
        \bottomrule
    \end{tabular}
    \caption{Performance comparison of VoteNet with and without our partially equivariant design on Scan2cad dataset (IoU=25\%).}
    \label{tbl:cmp_scan2cad}
\end{table*}

==> tbltext/cmp_waymo.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{c|cccccccccc|c}
        \toprule
        Method &  &  &  &  &  &  &  &  &  &  &  \\
        \hline
        CenterPoint~\cite{}  \\
        PE-CenterPoint (ours)  \\
        \bottomrule
    \end{tabular}
    \caption{Performance comparison of CenterPoint with and without our partially equivariant design on Waymo Open dataset (IoU=25\%).}
    \label{tbl:cmp_waymo}
\end{table*}

==> tbltext/rebut_abl_full_eqv.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lcc}
        \toprule
        Method & mAP@0.25 & mAP@0.5 \\
        \midrule
        FullEN-VoteNet &52.7 &26.9 \\
        \ourvn (ours) & \textbf{56.7} & \textbf{36.5} \\
        \bottomrule
    \end{tabular}
    \vspace{-0.2cm}
    \caption{Comparing full equivariance (denoted as ``FullEN-VoteNet'') with our object-level equivariance design on ScanNetV2 dataset with Scan2CAD detection labels.}
    \vspace{-0.2cm}
    \label{tbl:reb_abl_full_eqv}
\end{table}

==> tbltext/rebut_abl_layers.tex <==
\setlength{\columnsep}{5pt}
\begin{wraptable}{r}{.49\linewidth}
    \centering\vspace{-8pt}
    \setlength{\tabcolsep}{0pt}
    \scriptsize
    \begin{tabular}{lcc}
        \toprule
        Method & mAP@0.25 \\
        \midrule
        2nd-to-last backbone layer & 54.5 \\
        Last backbone layer & 54.2 \\
        Region aggregation (ours) & \textbf{56.7} \\
        Proposal & 52.7 \\
        \bottomrule
    \end{tabular}
    \vspace{-0.2cm}
    \caption{\footnotesize Suspension at various stages, for ObjEN-VoteNet on ScanNetV2 with Scan2CAD detection labels.}
    \vspace{-10pt}
    \label{tbl:reb_abl_layers}
\end{wraptable}

==> tbltext/rebut_category_pose.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lcc}
        \toprule
        Method & mAP@0.25 & mAP@0.5 \\
        \midrule
        VoteNet & 50.4 & 28.3 \\
        VoteNet+NOCS~\cite{wang2019normalized} &50.7 &28.5 \\
        ObjEN-VoteNet (ours) & \textbf{56.7} & \textbf{36.5} \\
        \bottomrule
    \end{tabular}
    \vspace{-0.2cm}
    \caption{Comparison to category-level pose estimation method on ScanNetV2 dataset with Scan2CAD detection labels.}
    \vspace{-0.2cm}
    \label{tbl:rebut_cat_pose}
\end{table}

==> tbltext/rebut_sota.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lcc}
        \toprule
        Method & mAP@0.25 & mAP@0.5 \\
        \midrule
        VoteNet & 50.4 & 28.3 \\
        Liu et.al.~\cite{liu2021} &53.5 &35.5 \\
        ObjEN-Liu et.al. (ours) & \textbf{61.4} & \textbf{44.9} \\
        \bottomrule
    \end{tabular}
    \vspace{-0.2cm}
    \caption{Comparison to a state-of-the-art method on ScanNetV2 dataset with Scan2CAD detection labels.}
    \vspace{-0.2cm}
    \label{tbl:rebut_sota}
\end{table}

==> tbltext/rebut_summary.tex <==
\begin{wraptable}{r}{.53\linewidth}
    \centering
    \scriptsize\vspace{-10pt}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{lcc}
        \toprule
        Method & mAP@0.25 & mAP@0.5 \\
        \midrule
        FullEN-VoteNet &52.7 &26.9 \\
        \midrule
        VoteNet & 50.4 & 28.3 \\
        VoteNet+NOCS~\cite{wang2019normalized} &50.7 &28.5 \\
        \ourvn (ours) & \textbf{56.7} & \textbf{36.5} \\
        \midrule
        Liu et.al.~\cite{liu2021} &53.5 &35.5 \\
        ObjEN-Liu et.al.(ours) & \textbf{61.4} & \textbf{44.9} \\
        \bottomrule
    \end{tabular}
    \vspace{-0.22cm}
    \caption{\footnotesize Results on ScanNetV2 with Scan2CAD detection labels.}
    \vspace{-0.4cm}
    \label{tbl:reb_summary}
\end{wraptable}
% \begin{table}[t]
%     \centering
%     \scriptsize
%     \begin{tabular}{lcc}
%         \toprule
%         Method & mAP@0.25 & mAP@0.5 \\
%         \midrule
%         FullEN-VoteNet &52.7 &26.9 \\
%         \midrule
%         VoteNet & 50.4 & 28.3 \\
%         VoteNet+NOCS~\cite{wang2019normalized} &50.7 &28.5 \\
%         \ourvn (ours) & \textbf{56.7} & \textbf{36.5} \\
%         \midrule
%         Liu et.al.~\cite{liu2021} &53.5 &35.5 \\
%         ObjEN-Liu et.al. (ours) & \textbf{61.4} & \textbf{44.9} \\
%         \bottomrule
%     \end{tabular}
%     \vspace{-0.2cm}
%     \caption{Results on ScanNetV2 with Scan2CAD detection labels.}
%     \vspace{-0.7cm}
%     \label{tbl:reb_summary}
% \end{table}

==> text/rebuttal_text.tex <==
We thank all reviewers for their constructive comments. %We respond to the questions below.

\myparagraph{R4, R5: Improving technical descriptions and presentations.} Thanks for this suggestion! Per \textbf{R5}'s suggestions, we have updated the notations in our main figure (Fig. \ref{fig:rebut_overview}), added them to section headers in the Method section, and associated technical descriptions (such as L422-L426 as \textbf{R4} pointed out) to the notations in figure to clarify them.

\myparagraph{R3, R4: Explanation for mixed results for indoor/outdoor scenes.} The object-level rotation equivariance is more useful when object orientations have a large variation, which is the case for indoor objects and pedestrians in outdoor scenes. Thus, our ObjEN design has significant performance gains on indoor scenes (e.g., $+6.3\%$ mAP on ScanNet) and pedestrians on KITTI (e.g., $+5.2\%$ AP on moderate difficulty). As for cars and cyclists, they are mostly axis-aligned with less orientation variations; thus, the performance gains are less significant. We will add this discussion to Sec. 5.3.

\myparagraph{R2, R3: Clarification on technical contributions.} Thanks for bringing this up. We propose a novel concept of object-level rotation equivariance in 3D scenes, which is technically \textbf{non-trivial} to obtain. 
% The challenge is how to maintain object-level equivariance while modeling context aggregation.
Directly applying existing equivariant designs to a detection pipeline cannot guarantee object-level rotation equivariance, as features are influenced by orientations of nearby objects
% We need an equivariance suspension mechanism since if we directly apply equivariant design to the whole detection network orientations of nearby objects can break object level equivariance
(``FullEN-VoteNet'' in Table~\ref{tbl:reb_summary}, taken from Table 5 in our main paper). We propose to suspend equivariance in an intermediate stage, but the challenge is how and where to execute suspension. We find it critical to suspend equivariance before region aggregation stage so that the context aggregation does not break object equivariance. We also find it important to differentiate objects and the background with the proposed orbit decomposition technique and to explicitly track the object frame; therefore, equivariance can be resumed for detection outcomes. Our \textbf{key technical contribution} is a novel and highly modular design reflecting these discoveries and allowing easy integration to existing detection networks. As also pointed out by \textbf{R5}, our technique is the first to enable extracting rotation-equivariant object features in 3D scenes, which we believe is significant. 
% \jw{I removed "for the first time".}

% If we simply break equivariance at an intermediate stage without resuming it, the design can't provide meaningful supervision to learn object-frame geometric features (Table \ref{}, taken from Table 1 in our supplementary material). Our technical contribution is the squivariance suspension design that allows maintaining object-level equivariance and resuming it on the detection outcomes.
% As \textbf{R5} pointed out, we are the first to overcome the technical challenges to enable extracting rotation-equivariant object features in 3D scenes, which is valuable for any kind of object-level analysis.
% extracting rotation-equivariant object features in 3D scenes is valuable for any kind of object-level analysis, and our approach is the first to overcome the technical challenge to enable extraction of such features in scene-level point clouds.
% In addition, our approach has a highly modular design to allow easy integration to existing detection networks.

\myparagraph{R2: Which intermediate stage to suspend equivariance?} 
\input{tbltext/rebut_abl_layers}%
This is a good question. Our approach assumes the input to region aggregation roughly corresponds to an object level, as the region aggregation stage (e.g., voting, RoI pooling, and map-view aggregation) typically aggregates context information for proposal generations. 
We verify our design on VoteNet by suspension at earlier (i.e., last few backbone layers) and  later stages (i.e., proposal stage).
Table~\ref{tbl:reb_abl_layers} shows that suspension at the input to region aggregation yields the best result. %Nevertheless, we agree that this is an important problem to further investigate in future work. 
We will include these results.

\input{figtext/overview_rebut}
\myparagraph{R2: Comparison to state-of-the-art.}
We apply our method to a transformer-based SOTA method from ICCV'21~\cite{liu2021}. We show results in Table~\ref{tbl:reb_summary}. While Liu et.~al.~\cite{liu2021} outperforms VoteNet, ours can further boost the performance. We will add this result to Sec. 5.2. We will also add visual results on SUN RGB-D and KITTI to our supplement.

% \myparagraph{R2: Visual results on SUN RGB-D and KITTI.}

\myparagraph{R2: Category-level pose estimation baseline.} We clarify that our equivariant design is not only to refine orientations. 
More importantly, it learns better geometric object features and distinguishes objects from backgrounds to improve proposal generations. Per your suggestion, \input{tbltext/rebut_summary}%
we attach a head to predict a NOCS~\cite{wang2019normalized} coordinate for each proposal, and use the estimated pose to refine object orientation.
Table~\ref{tbl:reb_summary} shows that category-level pose estimation can only marginally improve the baseline VoteNet.

\myparagraph{R2: ``Rotation symmetry'' in L17.} This means symmetry in networks rather than geometrically. We will replace it with ``rotation equivariance'' to avoid confusion.

\myparagraph{R4: Table 5 is important but overshadowed at the end of the paper.} Thank you. We agree and have moved it to the beginning of our Analysis section (5.4) with additional suspension variations shown in Table~\ref{tbl:reb_abl_layers}.

\myparagraph{R4: Why bin classification rather than regression for orientation?} 
It allows efficient implementation to decompose an equivariant feature orbit into an object-frame invariant feature and its orientation (we can use indexing to implement it). Also, it is more stable as pointed out in \cite{wang2019normalized}.

\myparagraph{R5: One rotation DoF in the datasets.} We choose to use 1 DoF because this is common due to gravity in detection scenarios. It is straightforward to extend our model to three DoFs. We've revised the limitation section as you suggested.

\myparagraph{R5: Performances of orientation classification.} On ScanNet, SUN RGB-D, and KITTI, the classification accuracy is 67.5\%, 69.0\%, and 95.1\%, respectively. As shown in Table 4 in the paper, using oracle orientations further improves detection performance.

%\input{tbltext/rebut_abl_layers}
% \input{tbltext/rebut_abl_full_eqv}
% \input{tbltext/rebut_sota}
% \input{tbltext/rebut_category_pose}
